MCVD: Masked Conditional Video Diffusion for Prediction, Generation, and Interpolation

Video prediction is a challenging task. The quality of video frames from current state-of-the-art (SOTA) generative models tends to be poor and generalization beyond the training data is difficult. Furthermore, existing prediction frameworks are typically not capable of simultaneously handling other video-related tasks such as unconditional generation or interpolation. In this work, we devise a general-purpose framework called Masked Conditional Video Diffusion (MCVD) for all of these video synthesis tasks using a probabilistic conditional score-based denoising diffusion model, conditioned on past and/or future frames. We train the model in a manner where we randomly and independently mask all the past frames or all the future frames. This novel but straightforward setup allows us to train a single model that is capable of executing a broad range of video tasks, specifically: future/past prediction -- when only future/past frames are masked; unconditional generation -- when both past and future frames are masked; and interpolation -- when neither past nor future frames are masked. Our experiments show that this approach can generate high-quality frames for diverse types of videos. Our MCVD models are built from simple non-recurrent 2D-convolutional architectures, conditioning on blocks of frames and generating blocks of frames. We generate videos of arbitrary lengths autoregressively in a block-wise manner. Our approach yields SOTA results across standard video prediction and interpolation benchmarks, with computation times for training models measured in 1-12 days using $\le$ 4 GPUs. Project page: https://mask-cond-video-diffusion.github.io ; Code : https://github.com/voletiv/mcvd-pytorch

==> FINAL_EXPS.tex <==
-----------------------------------------------------
PRED
-----------------------------------------------------

SMMNIST

smmnist_big_5c5_unetm_b2 - 700000
pred_fvd: 19.83094412352211
pred_fvd_conf95: 0.4556862235615071
pred_fvd_traj_mean: 25.634185095421447
pred_fvd_traj_std: 0.6974917301887735
pred_lpips: 0.11680526677228045
pred_mse: 0.023705631494522095
pred_psnr: 17.218151092529297
pred_ssim: 0.7856889094893715
preds_per_test: 10

DDPM_big_c5t5_SPADE - 140000
pred_fvd: 17.612452216697477
pred_fvd_conf95: 0.43836727783626017
pred_fvd_traj_mean: 23.863752456518124
pred_fvd_traj_std: 0.6709826526824672
pred_lpips: 0.12957946341630305
pred_mse: 0.024789508432149887
pred_psnr: 17.070545196533203
pred_ssim: 0.7803410298313221
preds_per_test: 10

--------------------------------

KTH

num_frames_pred = 40

DDPM_big_c10t5 - 100000
pred_fvd: 331.7369574154533
pred_fvd_conf95: 3.061584216234735
pred_fvd_traj_mean: 347.63682440552475
pred_fvd_traj_std: 4.686184399893276
pred_lpips: 0.11402942712884395
pred_mse: 0.0033832285553216934
pred_psnr: 25.727706909179688
pred_ssim: 0.6343741947900063
preds_per_test: 10

DDPM_big_c10t5_SPADE - 150000
pred_fvd_traj_mean: 314.6088380837646
pred_fvd_traj_std: 3.874396409687787
pred_lpips: 0.10999060848262161
pred_mse: 0.0032431045547127724
pred_psnr: 25.99102020263672
pred_ssim: 0.633148416046974
preds_per_test: 10

kth64_big_5c10_unetm_b2 - 400000
DDPM
----------
preds_per_test: 1
pred_lpips: 0.12883038006257266
pred_lpips_conf95: 0.0066510761631956156
pred_lpips_std: 0.054189347328140965
pred_mse: 0.003650873200967908
pred_mse_conf95: 0.0003844328072407808
pred_mse_std: 0.0031321493443101645
pred_psnr: 25.539363861083984
pred_psnr_conf95: 0.3961280433720802
pred_psnr_std: 3.22743558883667
pred_ssim: 0.7930666434659883
pred_ssim_conf95: 0.011145111138738395
pred_ssim_std: 0.09080429748343898
----------
DDPM
pred_fvd: 294.4330420619186
pred_fvd_conf95: 2.4849842790449657
pred_fvd_traj_mean: 308.05197085635075
pred_fvd_traj_std: 3.8036172582448224
pred_lpips: 0.10538705729413778
pred_mse: 0.0030784974806010723
pred_psnr: 26.268159866333008
pred_ssim: 0.6313130625517189
preds_per_test: 10
----------
DDIM
pred_fvd: 260.72969645599676
pred_fvd_conf95: 2.3772564733910713
pred_fvd_traj_mean: 276.6712497160309
pred_fvd_traj_std: 3.638724729856142
pred_lpips: 0.10590315015288071
pred_mse: 0.003099145134910941
pred_psnr: 26.19837188720703
pred_ssim: 0.6291717799684378
preds_per_test: 10
----------
DDIM
pred_lpips: 0.11129016904160381
pred_lpips_conf95: 0.005805763225703017
pred_lpips_std: 0.04730219775312401
pred_mse: 0.003253515111282468
pred_mse_conf95: 0.00035168641399016196
pred_mse_std: 0.002865349408239126
pred_psnr: 26.040382385253906
pred_psnr_conf95: 0.3912708368744582
pred_psnr_std: 3.187861680984497
pred_ssim: 0.8124371825527825
pred_ssim_conf95: 0.010548422092012566
pred_ssim_std: 0.0859428000044531
preds_per_test: 5

kth64_verybigbig_5c10_unetm_b2_spade - 340000
pred_fvd: 317.1118342102564
pred_fvd_conf95: 3.760857371206953
pred_fvd_traj_mean: 331.66835186237523
pred_fvd_traj_std: 5.75652012109224
pred_lpips: 0.10879234478343278
pred_mse: 0.0029910318553447723
pred_psnr: 26.397768020629883
pred_ssim: 0.6437552033849641
preds_per_test: 10

----------------------------------

num_frames_pred = 30

kth64_verybigbig_5c10_unetm_b2_spade - 340000
pred_fvd: 305.4386586922039
pred_fvd_conf95: 2.359339636699019
pred_fvd_traj_mean: 323.5362503144086
pred_fvd_traj_std: 3.6113004962987003
pred_lpips: 0.08678620234907915
pred_mse: 0.002376037882640958
pred_psnr: 27.512649536132812
pred_ssim: 0.6679819636958753
preds_per_test: 10
----------
pred_lpips: 0.08707925183698535
pred_lpips_conf95: 0.004618098268871676
pred_lpips_std: 0.03762575032175487
pred_mse: 0.00246474239975214
pred_mse_conf95: 0.0002407988389157528
pred_mse_std: 0.001961897825822234
pred_psnr: 27.38363265991211
pred_psnr_conf95: 0.4340206501104369
pred_psnr_std: 3.5361640453338623
pred_ssim: 0.834948707897675
pred_ssim_conf95: 0.010512229386188121
pred_ssim_std: 0.08564792154290128
preds_per_test: 10


-----------------------------------------------------
INTERP 
-----------------------------------------------------

SMMNIST

DDPM_interp_big_c5t10f5_SPADE - 125000
preds_per_test: 5
interp_lpips: 0.07094974687788635
interp_mse: 0.013850080780684948
interp_psnr: 19.567930221557617
interp_ssim: 0.8277272345668658
----------
preds_per_test: 100
interp_fvd: 37.80062285502001
interp_fvd_conf95: 0.31211574000113274
interp_fvd_traj_mean: 43.00443404307409
interp_fvd_traj_std: 1.5844742182710962
interp_lpips: 0.05612481778371148
interp_mse: 0.010136984288692474
interp_psnr: 20.944385528564453
interp_ssim: 0.8540616551579405

DDPM_interp_big_c5t5f5_SPADE - 150000
preds_per_test: 10
interp_lpips: 0.01664257819065824
interp_lpips_conf95: 0.0012624350737828697
interp_lpips_std: 0.010285633634900105
interp_mse: 0.0024265293031930923
interp_mse_conf95: 0.0003134642868815943
interp_mse_std: 0.0025539363268762827
interp_psnr: 27.693744659423828
interp_psnr_conf95: 0.42795841481062524
interp_psnr_std: 3.486772060394287
interp_ssim: 0.940977164036864
interp_ssim_conf95: 0.003750830619083545
interp_ssim_std: 0.030559725704432206

--------------------------------

KTH

DDPM_interp_big_c10t10f5_SPADE - 75000
preds_per_test: 5
interp_lpips: 0.03175379727908876
interp_mse: 0.0006933979457244277
interp_psnr: 33.728912353515625
interp_ssim: 0.7857293356643946
----------
preds_per_test: 10
interp_lpips: 0.030888345258426854
interp_lpips_conf95: 0.0020739133177897426
interp_lpips_std: 0.016897116549056155
interp_mse: 0.0006587360985577106
interp_mse_conf95: 8.521796917457768e-05
interp_mse_std: 0.0006943095941096544
interp_psnr: 34.06821823120117
interp_psnr_conf95: 0.5802658193887282
interp_psnr_std: 4.727689743041992
interp_ssim: 0.942145450775159
interp_ssim_conf95: 0.0051227739867805155
interp_ssim_std: 0.04173757329518199
----------
preds_per_test: 100
interp_lpips: 0.02886881438898854
interp_mse: 0.0005867546424269676
interp_psnr: 34.66934585571289
interp_ssim: 0.8159080046273057

DDPM_interp_big_c5t5f5_SPADE - 100000
preds_per_test: 10
interp_lpips: 0.020051980098651258
interp_lpips_conf95: 0.0014881467351762212
interp_lpips_std: 0.012124609360804199
interp_mse: 0.0003679495712276548
interp_mse_conf95: 3.803194041826312e-05
interp_mse_std: 0.00030986356432549655
interp_psnr: 35.611331939697266
interp_psnr_conf95: 0.40984662163241836
interp_psnr_std: 3.339207172393799
interp_ssim: 0.9628499434467302
interp_ssim_conf95: 0.0036393827114196142
interp_ssim_std: 0.02965170883179173


--------------------------------

BAIR

DDPM_PredPlusInterp_big_c1t5_SPADE - 50000




==> old_results.tex <==
% 10c5 unetm3d noisecond output_all_frames
% ckpt:150000, mse:0.4325334131717682, psnr:3.6399424076080322, ssim:0.0016844609402873547, % lpips:0.8055714111328125, fvd:1307.25732421875

% 10c5 unetm3d
% ckpt:150000, mse:0.4191661775112152, psnr:3.782240629196167, ssim:0.10412067035896322, lpips:0.7160143432617188, fvd:964.974365234375

% 10c5 unetmore 2blocks noisecond output_all_frames
% ckpt:450000, mse:0.4013778269290924, psnr:3.964520215988159, ssim:0.0007390324154366785, lpips:0.8168877563476562, fvd:1333.3238525390625

% 10c5 unet noisecond output_all_frames
% ckpt:550000, mse:0.41246211528778076, psnr:3.8462424278259277, ssim:0.0006017872309407698, lpips:0.8226683349609375, fvd:1282.3026123046875

% ###  5c5 stochastic mnist
% unetmore b1
% ckpt:100000, mse:0.03194069117307663, psnr:15.285572052001953, ssim:0.6841334242568451, lpips:0.22735659790039062, fvd:1212.463623046875
% normal
% ckpt:100000, mse:0.23418878018856049, psnr:6.379429817199707, ssim:0.2832983131965643, lpips:0.5933060302734375, fvd:708.9796142578125
% L1
% ckpt:100000, mse:0.0545790009200573, psnr:12.785849571228027, ssim:0.6291636829721935, lpips:0.3368864135742187, fvd:246.71316528320312
% unetmore b1 nhead=-1
% ckpt:100000, mse:0.05684112012386322, psnr:12.585762977600098, ssim:0.5978469665561139, lpips:0.34567971801757813, fvd:145.649658203125
% unetmore b1 L1
% ckpt:100000, mse:0.05228574573993683, psnr:12.973662376403809, ssim:0.6367174823797741, lpips:0.338866455078125, fvd:247.56301879882812
% unetmore b2
% ckpt:100000, mse:0.05330456793308258, psnr:12.935702323913574, ssim:0.6115297402357655, lpips:0.3181819152832031, fvd:109.69812774658203
% unetmore b1
% ckpt:100000, mse:0.05716206878423691, psnr:12.570086479187012, ssim:0.5963534777837971, lpips:0.34578298950195313, fvd:144.4368896484375
% gamma L1
% ckpt:100000, mse:0.0717041939496994, psnr:11.649428367614746, ssim:0.5784277454790792, lpips:0.3742270202636719, fvd:708.2650146484375
% gamma unetmore b2
% ckpt:100000, mse:0.056473538279533386, psnr:12.690834045410156, ssim:0.60477506298296, lpips:0.334482177734375, fvd:102.59127044677734
% gamma
% ckpt:100000, mse:0.28088971972465515, psnr:5.546575546264648, ssim:0.2251889414389306, lpips:0.6441217041015626, fvd:1359.6636962890625

%%% New Alexia 4/4/2022 

%%%% MNIST 5c5

%# unetmore ch=32 b1
%ckpt:100000, mse:0.057627420872449875, psnr:12.527826309204102, ssim:0.6002672859677669, lpips:0.33610174560546874, fvd:142.65084838867188
%ckpt:500000, mse:0.05383016914129257, psnr:12.962477684020996, ssim:0.623969696557677, lpips:0.31062423706054687, fvd:112.99240112304688
%ckpt:1000000, mse:0.05302898585796356, psnr:13.071834564208984, ssim:0.6246614514176508, lpips:0.318379150390625, fvd:119.68505096435547
%ckpt:1200000, mse:0.05345569923520088, psnr:12.907225608825684, ssim:0.6193816278438415, lpips:0.3218625793457031, fvd:84.49166870117188 *
%ckpt:1500000, mse:0.05270543694496155, psnr:12.98669719696045, ssim:0.6192160147717961, lpips:0.3210650634765625, fvd:113.4825439453125

%# unetmore ch=32 b2
%ckpt:100000, mse:0.054197486490011215, psnr:12.8829927444458, ssim:0.6143516508387048, lpips:0.31789642333984375, fvd:114.02827453613281
%ckpt:450000, mse:0.054005514830350876, psnr:12.919795036315918, ssim:0.6266690578127232, lpips:0.3072821655273438, fvd:89.0478286743164 *
%ckpt:500000, mse:0.05562296509742737, psnr:12.795785903930664, ssim:0.6138441028714406, lpips:0.32384878540039064, fvd:93.61430358886719
%ckpt:800000, mse:0.05649768188595772, psnr:12.742369651794434, ssim:0.6182444032876052, lpips:0.32082577514648436, fvd:99.06018829345703

%# unetmore ch=32 b1 L1
%ckpt:100000, mse:0.05223873630166054, psnr:12.991922378540039, ssim:0.6354510350406809, lpips:0.3389857177734375, fvd:288.2450866699219
%ckpt:500000, mse:0.05259852483868599, psnr:13.070396423339844, ssim:0.6422843991801319, lpips:0.3160479431152344, fvd:156.11695861816406
%ckpt:900000, mse:0.052475038915872574, psnr:13.10068130493164, ssim:0.6357436059487164, lpips:0.31801177978515627, fvd:115.58277130126953 *
%ckpt:1000000, mse:0.053029485046863556, psnr:13.094383239746094, ssim:0.6404705954075952, lpips:0.32257656860351563, fvd:136.755615234375
%ckpt:1150000, mse:0.05573330447077751, psnr:12.768306732177734, ssim:0.6256180223642736, lpips:0.3322208251953125, fvd:146.58070373535156

%# unetmore ch=32 b2 L1
%ckpt:100000, mse:0.051018908619880676, psnr:13.20268440246582, ssim:0.6441366886266221, lpips:0.31264459228515623, fvd:163.39077758789062
%ckpt:250000, mse:0.05138733237981796, psnr:13.138278007507324, ssim:0.6471420793685102, lpips:0.30914111328125, fvd:99.13760375976562 *
%ckpt:500000, mse:0.05318128690123558, psnr:13.017355918884277, ssim:0.6350769750121353, lpips:0.32093142700195315, fvd:104.11531066894531

%# unetmore gamma ch=32 b1
%ckpt:100000, mse:0.05936764180660248, psnr:12.454668045043945, ssim:0.5949348700737741, lpips:0.3344904479980469, fvd:155.29986572265625
%ckpt:500000, mse:0.05418604984879494, psnr:12.865021705627441, ssim:0.6193687719560962, lpips:0.32170556640625, fvd:118.781005859375
%ckpt:550000, mse:0.05419593304395676, psnr:12.86080551147461, ssim:0.620877562475994, lpips:0.3181943969726562, fvd:96.30180358886719
%ckpt:850000, mse:0.05515949800610542, psnr:12.780922889709473, ssim:0.6223155584531738, lpips:0.3086199645996094, fvd:93.28865814208984 *

%# unetmore gamma ch=32 b1 L1
%ckpt:100000, mse:0.05427338927984238, psnr:12.887245178222656, ssim:0.6301948799225914, lpips:0.34123873901367185, fvd:246.8256378173828
%ckpt:500000, mse:0.05004129931330681, psnr:13.259578704833984, ssim:0.6449536042056023, lpips:0.31800534057617186, fvd:178.5370635986328
%ckpt:700000, mse:0.055400922894477844, psnr:12.739522933959961, ssim:0.6277177148274061, lpips:0.3333991394042969, fvd:129.09083557128906 *

%# unetmore gamma ch=32 b2 L1
%ckpt:100000, mse:0.0540340431034565, psnr:12.908163070678711, ssim:0.6356962713266666, lpips:0.32618423461914064, fvd:179.21250915527344
%ckpt:500000, mse:0.05178013816475868, psnr:13.133166313171387, ssim:0.6442513865865541, lpips:0.31076318359375, fvd:131.12063598632812 
%ckpt:600000, mse:0.05399545654654503, psnr:12.96522331237793, ssim:0.6374856703760177, lpips:0.3160036926269531, fvd:98.40809631347656 *



%# unetmore3d ch=12
%ckpt:100000, mse:0.06008758395910263, psnr:12.382929801940918, ssim:0.5967289013393489, lpips:0.3347764587402344, fvd:191.98480224609375
%ckpt:300000, mse:0.05913536623120308, psnr:12.458745956420898, ssim:0.5972880876483698, lpips:0.32723370361328125, fvd:112.67623138427734 *
%ckpt:400000, mse:0.05594290792942047, psnr:12.675926208496094, ssim:0.6076959190862643, lpips:0.3310751647949219, fvd:126.79108428955078

%# unetmore3d ch=12 L1
%ckpt:100000, mse:0.05789114534854889, psnr:12.541496276855469, ssim:0.6301136106454478, lpips:0.36967532348632814, fvd:577.9121704101562
%ckpt:350000, mse:0.05821913853287697, psnr:12.519803047180176, ssim:0.6279602724778411, lpips:0.34842343139648435, fvd:294.4080810546875

%# unetmore3d gamma ch=12
%ckpt:100000, mse:0.06000985577702522, psnr:12.32366943359375, ssim:0.5879307886080999, lpips:0.3467556457519531, fvd:170.37197875976562
%ckpt:350000, mse:0.05636420100927353, psnr:12.629783630371094, ssim:0.6064817964335297, lpips:0.328674560546875, fvd:112.93063354492188 *
%ckpt:400000, mse:0.05478523299098015, psnr:12.746620178222656, ssim:0.6093241797291891, lpips:0.32879129028320314, fvd:119.6663589477539

%# unetmore3d gamma ch=12 L1
%ckpt:100000, mse:0.05600164458155632, psnr:12.638099670410156, ssim:0.6250353904819688, lpips:0.38047705078125, fvd:528.4682006835938
%ckpt:200000, mse:0.058080654591321945, psnr:12.558245658874512, ssim:0.6250153888354764, lpips:0.35997207641601564, fvd:417.00115966796875

%%%% MNIST 5c5

%# unetmore ch=32 b1
%ckpt:100000, mse:0.19203180074691772, psnr:7.16989278793335, ssim:0.009565161268417558, lpips:0.7370305786132813, fvd:7002.94287109375 *
%ckpt:1250000, mse:0.20157043635845184, psnr:6.958518028259277, ssim:0.009062841614106063, lpips:0.7260537719726563, fvd:7754.796875

%# unetmore ch=32 b2
%ckpt:100000, mse:0.1841004341840744, psnr:7.353021144866943, ssim:0.011598311709118377, lpips:0.7476773071289062, fvd:9168.9287109375
%ckpt:400000, mse:0.20288127660751343, psnr:6.930540084838867, ssim:0.008796233213473491, lpips:0.7309640502929687, fvd:6384.720703125 *

%# unetmore ch=32 b1 L1
%ckpt:100000, mse:0.11676932126283646, psnr:9.340365409851074, ssim:0.12816901139907116, lpips:0.6998115234375, fvd:7467.228515625
%ckpt:1350000, mse:0.117213174700737, psnr:9.320955276489258, ssim:0.12272135234994515, lpips:0.6762637939453126, fvd:6656.427734375 *

%# unetmore ch=32 b2 L1
%ckpt:100000, mse:0.11233220249414444, psnr:9.506928443908691, ssim:0.13531792637881976, lpips:0.7277735595703125, fvd:4785.23681640625
%ckpt:1100000, mse:0.11358822137117386, psnr:9.463168144226074, ssim:0.14852739196494838, lpips:0.6994024658203125, fvd:4302.27587890625 *

%# unetmore gamma ch=32 b1
%ckpt:100000, mse:0.1848996877670288, psnr:7.333805561065674, ssim:0.01014058114343082, lpips:0.7333129272460938, fvd:5568.00048828125 *
%ckpt:1300000, mse:0.20134280622005463, psnr:6.963555335998535, ssim:0.009381451629795673, lpips:0.7279698486328126, fvd:7641.96435546875

%# unetmore gamma ch=32 b1 L1
%ckpt:100000, mse:0.10717006772756577, psnr:9.713122367858887, ssim:0.08716469894116552, lpips:0.8031463623046875, fvd:4255.060546875
%ckpt:400000, mse:0.11010175943374634, psnr:9.609773635864258, ssim:0.09358235565802726, lpips:0.7886136474609375, fvd:4329.654296875 *

%# unetmore gamma ch=32 b2 L1
%ckpt:100000, mse:0.10719694197177887, psnr:9.722517013549805, ssim:0.13249601024939417, lpips:0.7457993774414062, fvd:5287.1552734375
%ckpt:600000, mse:0.10580144077539444, psnr:9.776723861694336, ssim:0.13474816316838883, lpips:0.7283302612304687, fvd:4893.330078125 *

